SNF-Bench: Separating Static Drift from Natural Flow in Long-Horizon Fixed-Camera Video Generation

Long-horizon video generation is evaluated with whole-frame metrics that reward motion and temporal consistency. For fixed-camera nature scenes this creates an ambiguity: motion of water, fire, smoke, or rain is desirable, whereas motion of the background is an error. A system can therefore score well on motion while its scene drifts, or on consistency while its flow stagnates. We introduce SNF-Bench, an evaluation framework for long-horizon fixed-camera generation that partitions each scene into static support and dynamic flow and reports static fidelity, flow persistence with absolute magnitude, and drift leakage separately, never as one score. Drift leakage is interpretive context rather than a headline measurement. Each factor is validated mechanistically rather than by correlation with preference: we inject global translation, rotation, and scale drift and progressive late freezing at known severity into real generations, and require each factor to respond in its stated direction and to remain selective against corruptions it does not target. Auditing publicly released long-horizon text-conditioned checkpoints under one recorded common inference configuration, plus an image-conditioned track with released-pipeline references and a deployment-sensitivity panel, we find that whole-frame motion and static-region drift induce near-opposite orderings of the same outputs. At maximum controlled translation, fBD and NBF rise to $1.86\times$ and $1.32\times$ baseline, but whole-frame Dynamic Degree reaches only $1.07\times$---rewarding the corruption. SNF-Bench measures where motion occurs and whether it persists; it does not measure physical realism. Project page: https://minar09.github.io/snfbench/.

==> generated/tab_perception.tex <==
\begin{table*}[tb]
\centering
\small
\setlength{\tabcolsep}{6pt}
\begin{tabular}{l l c c c c}
\toprule
Axis & Judge & agrees with factor & called indistinguishable & pairs & inter-rater $\alpha$ \\
\midrule
Static stability (fBD) & human & -- (3 decided) & -- & 8 & 0.18 \\
 & vision--language & -- (1 decided) & 1/1 & 7 & -- \\
Motion persistence (MCFF-L) & human & 4/5 decided pairs & -- & 8 & 0.24 \\
 & vision--language & -- (2 decided) & -- & 3 & -- \\
\bottomrule
\end{tabular}
\caption{\textbf{Perceptual pilot for the factor axes.} Each judge answers one question per axis and never which output is better. \emph{Agreement} is agreement with the factor's ordering on pairs the factor separates clearly, over pairs the judge decided; \emph{can't tell} is the share of near-tie pairs called indistinguishable, which is the correct answer there. The unit is the pair, majority-voted across raters. A dash marks a cell with too few decided pairs to carry a rate; the count is given instead. This exploratory protocol outcome is non-evidentiary, and no system is ranked by it.}
\label{tab:perception}
\end{table*}

==> sec/S14_perceptual.tex <==

\section{Exploratory Perceptual Pilot}
\label{sup:perceptual}

\textbf{This section supports no perceptual-validity claim.} It reports an
exploratory pilot that did not establish agreement between human judgments and
the factor orderings, and it is included because the reason it failed is
informative and because the protocol is what a powered study should start from.
Nothing here ranks systems, and no result from it enters any factor, table or
figure elsewhere in this work.

The pilot ran $24$ pairs per rater---twelve on each axis---with eight raters. After majority voting across raters, three pairs on the static axis and five on the persistence axis remained decided. Those counts, not the percentages they produce, are the honest summary of this run.

The question the pilot asked is whether independent judges order clip pairs the
way the factors do. That is metric validation rather than preference, so a small
sample would have been survivable had the pairs been constructed correctly; as
Sec.~\ref{sup:perceptual} reports below, they were not.

\paragraph{Ethics.}
Raters were volunteers drawn from the authors' institution and immediate
colleagues. Participation was voluntary and uncompensated, no personal data beyond a self-chosen identifier was collected, and no clip depicts an identifiable person. The study involved
no intervention and no sensitive material. Because a powered study will recruit
outside this group, we will obtain the institutional review or documented
exemption that such recruitment requires before running it.

\paragraph{Questions.}
One forced choice per axis, with an explicit third option:
\emph{static stability}---in which clip does the background stay more fixed in
place---and \emph{motion persistence}---in which clip does the intended motion
keep going rather than fade or freeze. Judges are never asked which output is
better, or which looks more natural. ``Better'' conflates the two failures the
benchmark separates, and naturalness is outside the stated scope, so either
question would produce a result the paper could not own.

\paragraph{Pairs.}
A pair is two systems' outputs on the \emph{same prompt at the same horizon},
never across prompts. Pairs are stratified by the relative gap in the axis's own
factor: \emph{clear-gap} pairs, where the factor separates the two outputs, carry
the agreement claim, while \emph{near-tie} pairs test the opposite property---that
where the factors do not separate, judges also cannot tell the clips apart.
Presentation side is randomized per trial and resolved back to a system
identity only after the response is recorded; system names are never shown.

\paragraph{Statistics.}
The unit of analysis is the pair, majority-voted across raters, and intervals
are percentile bootstrap resampling \emph{pairs}. Responses are clustered inside
rater and inside pair, so an interval computed over responses would claim
precision the design does not have. We report inter-rater agreement so the
reader can see whether the raters are signal or noise, and we run no
significance test the sample cannot power: the claim is descriptive agreement,
and saying so plainly is preferable to a $p$-value that would not survive
scrutiny.


\input{generated/tab_perception}

\paragraph{Outcome of the human arm: the protocol executed end to end.}
Eight raters each completed all $24$ trials. Engagement was genuine---median deliberation ran from $23$ to $233$ seconds per trial---and the ``can't tell'' option was used
deliberately, on $30\%$ of responses, rather than avoided.

The agreement estimate, however, does not survive its own error bars. Majority
voting across raters leaves three decided pairs on the static axis and five on
the persistence axis, and the corresponding intervals span most of the unit
range. Inter-rater agreement is low ($\alpha = 0.18$ and $0.24$ on the two
axes), and the direction of the estimate reverses depending on which rater
subset is used. We therefore report the counts and the interval rather than a
headline percentage, and we do not claim that perceptual agreement has been
established.

The cause is a property of the pair set rather than of the raters, and it is
measurable. The pairs were stratified by the gap in each axis's \emph{own}
factor but were not isolated against the other axis. On the static question the
median relative gap in the target factor is $0.29$ while the median gap in the
persistence factor is $0.58$: the clips shown differ about twice as much on the
axis the rater was told to ignore as on the one being asked about, and on half
the pairs both axes differ substantially. A rater seeing one clip drift and the
other stall cannot report which axis drove the answer, which is exactly the
condition that produces low inter-rater agreement and near-chance ordering. A
powered study therefore requires axis-isolated pairs---large gap in the target
factor, small gap in the other---and that constraint, not rater count, is the
first thing to fix.

\paragraph{Outcome of the vision--language arm: negative, with a located cause.}
The same pairs and the same wording were put to an open-weight
judge~\cite{qwen3vl2025} at temperature zero, each pair asked in both
presentation orders. Two controls precede any reading of its answers. Shown one
clip against itself, where the only correct answer is that they are the same, it
answered correctly on six of six. Shown a frozen single frame against a real
sequence---the largest difference available on the motion axis---its verdict
followed the swapped clip on only two of six. Presentation bias is absent: over
$48$ queries the two slots were chosen $8$ and $12$ times. The judge is
therefore well behaved and still cannot do the task: it answered
``indistinguishable'' on most pairs the factors separate clearly, leaving one
and two decided pairs on the two axes, which is far too few to support an
agreement rate. We report none.

The controls locate the cause in the judge rather than in the factors or the
prompt. A model that cannot separate a still image from moving water is not
positioned to separate two rollouts that differ subtly. This says that an
open-weight judge at this scale cannot presently substitute for human raters on
these axes. It does not say that stronger judges would fail, and we make no
claim about them: contemporary generation benchmarks that report successful
automated judging use frontier proprietary
models~\cite{han2025videobench,sun2024t2v_compbench} or scorers fine-tuned for
the task~\cite{he2024videoscore}, and we have no evidence either way about those
here.

\paragraph{Status.}
Both arms are exploratory and support no agreement claim. The protocol executed end to end, but the resulting judgments were too sparse and inconsistent to support perceptual validation, that raters engage with the axis questions rather than defaulting to a side, and that the binding constraint on a powered study is pair construction rather than rater count: axis-isolated pairs, and a near-tie stratum. Protocol, pair manifest and judge prompt are released verbatim so the check can be repeated and enlarged. To restate the scope without qualification: what is released here is a documented, executable \emph{protocol} and a diagnosis of why this run of it failed. \textbf{No conclusion about
perceptual agreement, in either direction, should be drawn from the counts in
this section.} They are reported so the pilot is auditable, not because they
support an inference.

